Cross-System Categorization of Abnormal Traces in Microservice-Based Systems via Meta-Learning

Microservice-based systems (MSS) may fail with various fault types. While existing AIOps methods excel at detecting abnormal traces and locating the responsible service(s), human efforts are still required for diagnosing specific fault types and failure causes.This paper presents TraFaultDia, a novel AIOps framework to automatically classify abnormal traces into fault categories for MSS. We treat the classification process as a series of multi-class classification tasks, where each task represents an attempt to classify abnormal traces into specific fault categories for a MSS. TraFaultDia leverages meta-learning to train on several abnormal trace classification tasks with a few labeled instances from a MSS, enabling quick adaptation to new, unseen abnormal trace classification tasks with a few labeled instances across MSS. TraFaultDia's use cases are scalable depending on how fault categories are built from anomalies within MSS. We evaluated TraFaultDia on two MSS, TrainTicket and OnlineBoutique, with open datasets where each fault category is linked to faulty system components (service/pod) and a root cause. TraFaultDia automatically classifies abnormal traces into these fault categories, thus enabling the automatic identification of faulty system components and root causes without manual analysis. TraFaultDia achieves 93.26% and 85.20% accuracy on 50 new classification tasks for TrainTicket and OnlineBoutique, respectively, when trained within the same MSS with 10 labeled instances per category. In the cross-system context, when TraFaultDia is applied to a MSS different from the one it is trained on, TraFaultDia gets an average accuracy of 92.19% and 84.77% for the same set of 50 new, unseen abnormal trace classification tasks of the respective systems, also with 10 labeled instances provided for each fault category per task in each system.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/evaluation0209.tex <==
\section{Evaluation}
% To evaluate our model, we defined these research questions: 
% \begin{itemize}
%     \item  \textbf{RQ1: Within-system adaptability}. How effective is our framework, once trained on abnormal trace classification tasks within a MS, can adapt to novel, previously unseen tasks within the same MS?

%     \item  \textbf{RQ2: Cross-system adaptability.} How effective is our framework, once trained on abnormal trace classification tasks within a MS, can adapt to novel, previously unseen tasks in a different MS?
%     \Serge{Is this unseen tasks? Or is this coss project training?}

%     \item \textbf{RQ3: Component Impact.} How does each component of our framework contribute to its overall performance?
%     \Serge{I am not convinced of this ablation study. It feels like you want to do something with the data because you have it. Why is this necessary for a proof-of-concept lkike this?}
% \end{itemize}

\subsection{Experimental design}
\label{sec:ex_design}
\subsubsection{Dataset} To train and evaluate our framework, we use trace data of TrainTicket and OnlineBoutique from DeepTraLog and Nezha. Detailed descriptions of these MSS and open datasets have been presented in Section \ref{sec:emprical_study}. As described in Section \ref{sec:emprical_study}, we establish our fault dataset (using DeepTraLog and Nezha), which includes abnormal traces from 30 fault categories for TrainTicket and 32 fault categories for OnlineBoutique. For our experiments, we further operate our fault dataset.  We divide 30 fault categories of Trainticket into 20 base and 10 novel fault categories, and 32 fault categories of OnlineBoutique into 22 base and 10 novel fault categories. Fault categories within each system do not overlap. That is, there are 20 and 22 base fault categories in TrainTicket and OnlineBoutique, respectively, along with 10 novel fault categories for each system. To provide a consistent basis to compare experimental results, we standardized the number of novel fault categories for both systems. We design the composition of both base and novel fault categories for each system to include a random mix of fault categories from our dataset. This mix incorporates fault categories that comprise traces with varying lengths of spans and logs. It ensures the representation of fault categories with abnormal traces containing both short and long spans and logs within base and novel fault categories for each system. The full list of base and novel fault categories for each system is provided in our replication package.

\subsubsection{Training and evaluation} 
\label{sec:evaluation:training} Our training and evaluation process is designed based on our framework workflow (Section \ref{sec:ourFrameworkDesign}). We utilize a random selection of 3960 normal traces (3360 training/570 validation) from each MSS, TrainTicket and OnlineBoutique respectively, to train AttenAE to construct compact yet effective trace representations tailored to each MSS.


To train and evaluate TEMAML, we use our fault dataset, which includes 20 and 22 base fault categories for TrainTicket and OnlineBoutique respectively, and 10 novel fault categories for each MSS. For each MSS, we randomly generate 4 meta-training tasks using its base fault categories, and 50 meta-testing tasks using its novel fault categories. Considering prior meta-learning studies~\cite{ye2021train,finn2017model} and the constraint of our fault dataset, we configure each meta-training task $T_{i}$ and each meta-testing task $T_{ts}$ in 5-way 5-shot and 5-way 10-shot setups. Each $T_{i}$ and $T_{ts}$ is a distinct abnormal trace classification task with 5 fault categories, each category has 5/10 labeled trace instances as the support set ($T_{i}$, $T_{ts}$=5/10) for fine-tuning TEMAML to this task. For each $T_{i}$ and $T_{ts}$, we evaluate TEMAML on the query set consisting of 15 trace instances per fault category ($Q_{i}, Q_{ts}$=15). Specifically, for each MSS, we generate 4 meta-training tasks by performing 4 iterations of selecting a unique permutation of 5 fault categories from this MSS's base fault categories, and 50 meta-testing tasks by performing 50 iterations of selecting a unique permutation of 5 fault categories from this MSS's novel fault categories. The number of unique permutations for selecting 5 out of 10 novel fault categories is 252. We focus on 50 distinct meta-testing tasks, representing about 20\% of 252 unique permutations, to evaluate our framework, following the prior studies \cite{ye2021train,finn2017model}. This approach allows for a focused comprehensive evaluation, ensuring a broad coverage of various fault categories while keeping the data size within practical limits. For each MSS, TEMAML uses the optimized AttenAE’s encoder for this MSS to construct compact trace representations for abnormal traces in each MSS's meta-training and meta-testing tasks. With meta-training and meta-testing tasks for both MSS, we design four experiments E1-E4. E1 and E2 are within-system experiments for RQ1, while E3 and E4 are cross-system experiments for RQ2:  
\begin{itemize}
    \item \textbf {E1 (TrainTicket→TrainTicket).} We train TEMAML on TrainTicket's 4 meta-training tasks and evaluate it on TrainTicket's 50 meta-testing tasks. 
    \item \textbf{E2 (OnlineBoutique→OnlineBoutique).} We train TEMAML on OnlineBoutique's 4 meta-training tasks and evaluate it on OnlineBoutique's 50 meta-testing tasks. 
   \textbf{ \item E3 (OnlineBoutique→TrainTicket).} We train TEMAML on OnlineBoutique's 4 meta-training tasks and evaluate it on  TrainTicket's 50 meta-testing tasks. 
    \textbf{ \item E4 (TrainTicket→OnlineBoutique).} We train TEMAML on TrainTicket's 4 meta-training tasks and evaluate it on  OnlineBoutique's 50 meta-testing tasks. 
\end{itemize}

% \begin{table}
% \centering
% \caption{Descriptive statistics on traces in our fault dataset.}
% \label{tab:dataset_trace_statistics}
% \begin{tabular}{lrrr}
% \toprule
% \textbf{Trainticket.Base fault categories} & Mean & Min & Max  \\
% Unique traces per fault category: & 1117 & 26 & 2309  \\
% Spans per trace: & 71 & 1 & 303 \\
% Logs per trace: & 44 & 1 & 219 \\ \hline

% \textbf{Trainticket.Novel fault categories} & Meam & Min & Max  \\
% Unique traces per fault category: & 1275 & 45 & 2546  \\
% Spans per trace: & 87 &  1 & 345  \\
% Logs per trace: & 60 & 1 & 340 \\ \hline

% \textbf{OnlineBoutique.Base fault categories} & Mean & Min & Max  \\
% Unique traces per fault category: & 565 & 32 & 1018  \\
% Spans per trace: & 53 & 1& 180 \\
% Logs per trace : & 53 & 4  & 184  \\ \hline

% \textbf{OnlineBoutique.Novel fault categories} & Mean & Min & Max  \\
% Unique traces per fault category: & 320 & 34 & 902  \\
% Spans per trace: & 52  & 1 &  190\\
% Logs per trace: &  49 & 4 & 164  \\
% \bottomrule
% \end{tabular}
% \end{table}


\subsubsection{Implementation details} E1-E4 are conducted on a Linux server with a 32-core CPU and an NVIDIA Ampere A100 GPU with 40 GB of memory, utilizing Python 3.10.6.  We train AttenAE and TEMAML using the AdamW optimizer. Further details regarding hyperparameter settings of AttenAE and TEMAML are provided in our replication package.

\subsubsection{Baselines}
\label{sec:baselines} We considered prior trace representation and classification methods to build our baselines. We combine baselines with ablation studies to systematically explore alternatives to evaluate the performance of our framework and the impact of each components within it:

\begin{table}[!ht]
\centering
\small
\label{tab:baselines}
%\caption{Baselines.}
%\vspace{-10pt}
\begin{tabular}{l}
\hline
\textit{AttenAE alternative:} \\
Feed \textbf{only spans (OnlySpan)} into TE-MAML for classification. \\

\textit{Multihead atten fusion alternatives:}\\
\textbf{Linear-based AE (LinearAE) fusion +TEMAML} \\
\textbf{Gated linear unit-based AE (GluAE) fusion +TEMAML } \\

\textit{TE alternatives:} \\
   AttenAE+\textbf{LinearMAML} \\
   AttenAE+\textbf{RnnMAML} \\
   AttenAE+\textbf{LstmMAML}\\
   AttenAE+\textbf{CnnMAML}\\

\textit{MAML alternatives:} \\
    AttenAE+\textbf{Prototypical network (ProtoNet)}   \\
    AttenAE+\textbf{TE-based Matching network (TE-MatchNet)} \\
    AttenAE+\textbf{Nearest neighbor (NNeighbor)}  \\
    AttenAE+\textbf{Decison tree (DTree)}\\
\hline
\end{tabular}

\vspace{-10pt}
\end{table}


AttenAE and multihead attention fusion alternatives incorporate different approaches than ours for constructing trace representations. The baseline OnlySpan follows the related work~\cite{nedelkoski2019anomaly2} to consider each trace as a sequence of spans and construct trace representations using only span attributes. GluAE uses gated linear units to construct trace representations by fusing the same span and log attributes as our framework, modified from the modality fusion method for MSS in the study~\cite{lee2023eadro}. LinearAE is a simplified version of GluAE, utilizing linear projection to do fusion without the gating mechanism. 

We consider many TE alternatives, including the basic linear model, sequence models (RNN and LSTM), and CNN, as the alternative base models to perform multi-class classification on abnormal traces. We include sequence models here because prior studies \cite{kohyarnejadfard2019system,zhang2022putracead} have shown their effectiveness in performing binary classifications for normal and abnormal traces. CNN was considered as it has been used in related work~\cite{nedelkoski2019anomaly2} to do multi-class abnormal trace classification. The basic linear model serves as a simplest approach for evaluation. 


MAML alternatives use other meta-learning methods (Prototypical network  \cite{snell2017prototypical}, matching network \cite{vinyals2016matching}) and traditional models (Nearest neighbor and Decision tree) for multi-class classification of abnormal traces. These alternatives completely replace our use of MAML algorithm, exploring different efficient strategies to handle abnormal trace classification tasks. Since the fundamental machine learning models used in these alternatives are simple and do not support transfer learning (i.e., cross-system adaptability), we only evaluate these alternatives on E1 and E2. For each meta-testing task $T_{ts}$ in E1 and E3, we train each MAML alternative using this task's support instances $S_{ts}$, and then evaluate them on this task's query instances $Q_{ts}$. The motivation for using these baselines is: if they can categorize abnormal traces efficiently and effectively with limited number of labeled traces as our framework, transfer learning may not be necessary for them.

We use the same neural representation method \cite{le2021log} as in our framework to handle textual span and log attributes in all baselines, although some of the previous studies referenced in our baselines utilized parsing and template approaches. The purpose is to ensure a fair comparison and demonstrate that the performance of our framework does not solely stem from the use of neural representations. This decision is driven by an empirical study \cite{le2021log}, which shows that neural representations are more effective at capturing the semantic meaning of textual log data.

\subsubsection{Evaluation metrics} 
To evaluate \textbf{adaptation effectiveness} of our framework and baselines, we chose accuracy as the evaluation metric, a standard measure for multi-class classification tasks. Accuracy may not be the ideal metric in contexts where the distribution of classes is uneven. For instance, in anomaly detection-related binary classification tasks, normal traces often significantly outnumber abnormal ones, and a model could achieve high accuracy simply by predicting the most frequent class—normal traces. However, accuracy is suitable for our study as we perform multi-class classification tasks on already detected abnormal traces within a 5-way meta-learning setup in each experiment. This setup ensures that consistently predicting a single class would yield a maximum accuracy of only 20\%. Using accuracy aligns with prior meta-learning studies \cite{finn2017model,ye2021train} on multi-class classification using accuracy as the only metric. Therefore, accuracy is the most suitable metric to evalaute the effectiveness of our framework and baselines in accurately classifying abnormal traces into diverse fault categories. To mitigate the risk of obtaining an inaccurate evaluation of the approach's effectiveness, in each experiment, we calculate the accuracy for each meta-testing task by conducting five trials and selecting the highest accuracy achieved. As evaluation results, we report the average accuracy along with the 95\% confidence interval (CI) computed across 50 meta-testing tasks in each experiment, as well as the range of task accuracies (minimum and maximum). This provides a comprehensive view of the approach's effectiveness and offers insights into its consistency and reliability in various scenarios. Besides, we perform t-tests~\cite{fisher1970statistical} to statistically compare the accuracy of our framework with effective baselines across 50 meta-testing tasks in each experiment.  We further quantify the differences using 
 Cohen's D value to assess the effect size. According to Cohen ~\cite{cohen2013statistical}, a value of 0.2 indicates a small effect size, 0.5 signifies a medium effect size, and 0.8 or higher denotes a large effect size.
 
 %to compare the effect size of our framework with effective baselines, quantifying the differences in performance. We interpret Cohen's D values using the common standard as follows: 0.2 indicates a small effect size, 0.5 signifies a medium effect size, and 0.8 or higher denotes a large effect size. We interpret Cohen's D values using the standard~\cite{cohen2013statistical}: 0.2 indicates a small effect size, 0.5 signifies a medium effect size, and 0.8 or higher denotes a large effect size.

We compare \textbf{adaptation efficiency} of our framework with effective baselines in our experiments. We calculate the time each approach takes during the meta-testing phase, focusing on two key aspects: the average adaptation time for each meta-testing task, and the average time required to construct trace representations for each meta-testing task.

\subsection{Experiment results}
\textbf{Adaptation effectiveness.} Table \ref{tab:E1_Result}-\ref{tab:E4_Results} shows the average accuracy (in \%) with the corresponding 95\% confidence interval, computed across 50 meta-testing tasks in each experiment. Our TraFaultDia demonstrates high accuracy on 50 meta-testing tasks for each experiment in both the 5-shot and 10-shot setups, indicating its effectiveness in both within-system and across-system adaptability. Compared to other effective baselines, our framework demonstrates better robustness. Specifically, the "GluAE +TEMAML" and "GluAE +ProtoNet" methods achieve similar accuracy to our framework in E1 and E3 setups, however, their accuracy is lower by around 2\%-9\% and 6\%-10\% respectively in E2 and E4 setups; "AttenAE+CnnMAML" achieve around 79.01-84.08\% accuracy from E2 and E4 setups, but only obtain 49.04-69.20\% accuracy from E1 and E3 setups. Besides, though "AttenAE+NNeighbor" lacks cross-system adaptability (NNeighbor has no transfer learning ability), it only achieves about 1\%-4\% lower average accuracy to our framework in E1 and E2 setups concerning within-system adaptability for Tracintikcet and OnlineBoutique respectively. 

Table \ref{tab:t_tests} presents t-test results of accuracy on 50 meta-testing tasks in each experiment, comparing our framework to the top three effective baselines (see Table \ref{tab:E1_Result}-\ref{tab:E4_Results}) in all experiment setups. Except for GluAE+TEMAML in the E1 setups (5-shot and 10-shot) and AttenAE+NNeighbor in the E2 10-shot setup, our TraFaultDia demonstrates significant differences from the three baselines (p < 0.05) in all other E1-E4 setups. Table \ref{tab:effectSize} compares Cohen's D values of the accuracy of our framework to these baselines across 50 meta-testing tasks in each experiment. Our framework demonstrates large positive effect sizes (Cohen's D > 0.8) against GluAE+TEMAML primarily in E2 and E4, and against LinearAE+TEMAML and AttenAE+NNeighbor in all 5-shot setups across the experiments. The above t-test results and effect size measurements provide strong evidence for the effectiveness of our framework over these three baselines.


\begin{table}[!ht]
\centering
\small
\caption{\textbf{E1 (TrainTicket→TrainTicket}). Accuracy, 95\% CI and min-max: train on TrainTicket's 4 meta-training tasks and adapt to TrainTicket’s 50 meta-testing tasks.}
\label{tab:E1_Result}
\begin{tabular}{p{4cm}p{4cm}p{4cm}}
\toprule
Framework & 5-shot & 10-shot \\
\midrule
\textbf{Our TraFaultDia} & 92.91$\pm$2.10 (74.67-100.0) & 93.26$\pm$1.40 (76.00-100.0)\\
\textit{AttenAE alternatives:}& & \\
\textbf{OnlySpan}+TEMAML & 80.64$\pm$2.84 (57.33-97.33) &  78.77$\pm$2.80 (60.00-97.33)\\
% ... 其他行 ...

\multicolumn{2}{l}{\textit{Multihead atten fusion alternatives:}} & \\
%\textit{Multihead atten fusion alternatives:}& & \\
\textbf{LinearAE}+TEMAML &  89.15$\pm$2.29  (73.33-100.0)&  90.59$\pm$2.43 (70.67-100.0) \\
\textbf{GluAE }+TEMAML & 92.21$\pm$1.73  (77.33-100.0) & 93.07$\pm$1.64 (77.33-100.0) \\

%92.21$\pm$1.73  (77.33-100.0) & 93.07$\pm$1.64 (77.33-100.0) & 85.07$\pm$2.38 (66.67-100.0) & 94.40$\pm$2.19 (72.00-100.0)  \\

\multicolumn{2}{l}{\textit{Transformer encoder alternatives:}}& \\
AttenAE+\textbf{LinearMAML} &  45.84$\pm$2.21 (25.33-61.33) &  45.36$\pm$2.16 (30.67-60.00) \\
AttenAE+\textbf{RnnMAML}  & 49.65$\pm$2.09 (37.33-64.00) & 42.88$\pm$1.93 (24.00-58.67) \\
AttenAE+\textbf{LstmMAML}  & 41.39$\pm$2.20 (21.33-56.00) & 42.67$\pm$1.91 (29.33-56.00)   \\
AttenAE+\textbf{CnnMAML}  & 57.06$\pm$2.85 (41.33-81.00) & 69.20$\pm$2.19 (56.00-88.00) \\ 

\textit{MAML alternatives:}& &  \\
AttenAE+\textbf{TEMatchNet}  & 76.56$\pm$2.80 (49.33-93.33) & 76.05$\pm$2.37 (50.67-94.67)  \\
AttenAE+\textbf{ProtoNe}t & 57.25$\pm$0.03 (40.00-74.67) & 59.68$\pm$0.03 (44.00-76.00)   \\
AttenAE+\textbf{NNeighbor} & 88.19$\pm$0.02 (74.67-98.67) & 92.56$\pm$0.02 (78.00-100.0)  \\
%MultiHAttenAE+\textbf{RelationNet}  &  &  &  &   \\
AttenAE+\textbf{DTree}  & 66.80$\pm$0.03 (46.67-88.00) & 77.09$\pm$0.03 (54.67-96.00)   \\

\bottomrule
\end{tabular}
\end{table}

\begin{table}[!ht]
\centering
\small
\caption{ \textbf{E2 (OnlineBoutique→OnlineBoutique)}. Accuracy, 95\% CI and min-max: train on OnlineBoutique's 4 meta-training tasks and adapt to OnlineBoutique's 50 meta-testing tasks. }
\label{tab:E3.Results}
%\begin{tabular}{lllll}
\begin{tabular}{p{4.1cm}p{4cm}p{4cm}}
\toprule
% Header row
Framework & 5-shot & 10-shot \\
\midrule

\textbf{Our TraFaultDia}  & 82.50$\pm$2.35 (65.33-98.67) & 85.20$\pm$2.33 (66.67-98.67)  \\ 

\textit{AttenAE alternatives:}& &\\

\textbf{OnlySpan}+TE-MAML & 72.83$\pm$2.40 (57.33-88.00) & 73.15$\pm$2.81 (46.67-92.00) \\
% ... 其他行 ...
\multicolumn{2}{l}{\textit{Multihead atten fusion alternatives:}} & \\
\textbf{LinearAE}+TE-MAML & 76.15$\pm$2.59 (60.00-95.00) & 78.21$\pm$2.50 (64.00-96.00) \\
\textbf{GluAE }+TE-MAML  & 80.61$\pm$2.96 (58.67-98.67) & 77.49$\pm$2.67 (48.00-94.67) \\

\multicolumn{2}{l}{\textit{Transformer encoder alternatives:}} &  \\
 AttenAE+\textbf{LinearMAML} & 42.59$\pm$3.63 (20.00-77.33)  &  40.75$\pm$3.53 (21.33-68.00)\\
 AttenAE+\textbf{RnnMAML}  &  72.59$\pm$2.50 (54.67-94.67) & 64.75$\pm$2.53 (46.67-80.00) \\
 AttenAE+\textbf{LstmMAML}  & 54.80$\pm$2.11 (40.00-70.67) & 55.97$\pm$2.25 (41.33-69.33) \\ 
AttenAE+\textbf{CnnMAML}  & 80.10$\pm$2.16 (60.00-94.67) & 83.07$\pm$3.29 (68.00-97.33) \\ 

\textit{MAML alternatives:}& & \\
AttenAE+\textbf{TEMatchNet} & 76.29$\pm$3.00 (54.67-96.00) & 73.11$\pm$2.94 (50.67-94.67)  \\
AttenAE+\textbf{ProtoNet} & 74.51$\pm$0.03 (53.33-92.00) & 76.59$\pm$0.04 (58.66-94.67)  \\
AttenAE+\textbf{NNeighbor} & 80.96$\pm$0.03 (64.00-98.67) & 84.75$\pm$0.03 (62.80-98.67) \\

%MultiHAttenAE+\textbf{RelationNet}  &  &  &  &   \\
AttenAE+\textbf{DTree}  &  66.99$\pm$0.02 (54.67-80.00) & 73.79$\pm$0.03 (58.67-82.67)  \\

\bottomrule
\end{tabular}
\end{table}

\begin{table}[!ht]
\centering
\small
\caption{ \textbf{E3 (OnlineBoutique→TrainTicket).} Accuracy, 95\% CI and min-max: train on OnlineBoutique's 4 meta-training tasks and adapt to TrainTicket's 50 meta-testing tasks.}
\label{tab:E2_Result}
\begin{tabular}{p{4.1cm}p{4cm}p{4cm}}
\toprule
% Header row
Framework & 5-shot & 10-shot \\
\midrule
\textbf{Our TraFaultDia} & 86.35$\pm$2.00 (70.67-100.0) & 92.19$\pm$1.99 (74.67-100.0)\\
\textit{AttenAE alternatives:}& &  \\
\textbf{OnlySpan}+TEMAML & 79.25$\pm$2.89 (57.33-97.33) & 80.19$\pm$3.10 (56.00-97.33)\\
% ... 其他行 ...
\multicolumn{2}{l}{\textit{Multihead atten fusion alternatives:}}&\\
\textbf{LinearAE}+TEMAML &   83.09$\pm$2.55 (62.67-97.33) & 90.61$\pm$2.01  (72.00-100.0) \\
\textbf{GluAE }+TEMAML & 85.07$\pm$2.38 (66.67-100.0) & 94.40$\pm$2.19 (72.00-100.0)  \\

%92.21$\pm$1.73  (77.33-100.0) & 93.07$\pm$1.64 (77.33-100.0) & 85.07$\pm$2.38 (66.67-100.0) & 94.40$\pm$2.19 (72.00-100.0)  \\

\multicolumn{2}{l}{\textit{Transformer encoder alternatives:}}& \\
 AttenAE+\textbf{LinearMAML} & 43.81$\pm$1.99 (28.00-58.67) &  43.87$\pm$1.93 (29.33-60.00) \\
 AttenAE+\textbf{RnnMAML}  & 48.45$\pm$1.75 (38.67-65.33) & 47.07$\pm$1.88 (34.67-58.67)\\
 AttenAE+\textbf{LstmMAML}  & 40.32$\pm$1.68 (22.67-52.00) & 42.29$\pm$1.79 (25.33-56.00)  \\
 AttenAE+\textbf{CnnMAML}  & 49.04$\pm$1.80 (38.67-64.00) & 69.47$\pm$2.65 (48.00-89.33)\\ 

\bottomrule
\end{tabular}
\end{table}


\begin{table}[!ht]
\centering
\small
\caption{ \textbf{E4 (TrainTicket→OnlineBoutique).} Accuracy, 95\% CI and min-max: train on TrainTicket's 4 meta-training tasks and adapt to OnlineBoutique's 50 meta-testing tasks. }
\label{tab:E4_Results}
%\begin{tabular}{lllll}
\begin{tabular}{p{4.1cm}p{4cm}p{4cm}}
\hline
% Header row
Framework& 5-shot & 10-shot \\
\midrule

\textbf{Our TraFaultDia} & 82.37$\pm$2.07 (64.00-97.33) & 84.77$\pm$2.28 (68.00-98.67) \\ 

\multicolumn{2}{l}{\textit{AttenAE alternatives:}}&  \\

\textbf{OnlySpan}+TE-MAML &  71.81$\pm$2.25 (56.00-85.33) &  73.60$\pm$2.21 (57.33-85.33)\\
% ... 其他行 ...
\multicolumn{2}{l}{\textit{Multihead atten fusion alternatives:}} & \\
\textbf{LinearAE}+TEMAML &  75.81$\pm$2.45 (52.00-89.33) &  74.32$\pm$2.44 (53.33-88.00)\\
\textbf{GluAE }+TEMAML & 74.96$\pm$2.76 (54.67-94.67) & 77.57$\pm$2.7 (56.00-94.67)\\

\multicolumn{2}{l}{\textit{Transformer-encoder alternatives:}} &\\
 AttenAE+\textbf{LinearMAML} & 47.01$\pm$3.59 (25.33-74.67) & 44.35$\pm$4.10 (20.00-89.33)  \\
 AttenAE+\textbf{RnnMAML} & 72.58$\pm$2.58 (54.70-94.70) & 71.01$\pm$2.80 (56.00-89.33) \\
 AttenAE+\textbf{LstmMAML} & 56.19$\pm$1.92 (38.67-72.00) & 59.71$\pm$2.05 (42.67-77.33) \\ 
 AttenAE+\textbf{CnnMAML} & 79.01$\pm$2.63 (56.00-97.33) & 84.08$\pm$2.76 (65.33-100.0) \\ 

\hline
\end{tabular}
\end{table}



\begin{table}[!ht]
\centering
\small
\caption{T-test results of accuracy, comparing Our TraFaultDia to  effective baselines }
\label{tab:t_tests}
\begin{tabular}{p{3.2cm} | p{0.35cm} p{1.6cm}  p{1.6cm} | p{0.35cm} p{1.6cm} p{1.6cm}}
\hline
% Header row
 %& \multicolumn{2}{c}{E1} & \multicolumn{2}{c}{E3} \\
 %\cmidrule(l){2-5}
% Sub-header row
\textbf{Our TraFaultDia v.s.} & E1 & 5-shot & 10-shot & E3 & 5-shot & 10-shot\\ \hline 
 
GluAE+TEMAML & & 0.0719 & 0.5347 & & 0.0045*** & 7.74e-07*** \\
LinearAE+TEMAML & & 1.62e-13*** %1.62 \times 10^{-13} 
& 1.14e-09*** %1.14\times 10^{-9} 
& & 1.87e-10*** & 0.0005*** \\
AttenAE+NNeighbor & & %$7.10 \times 10^{-29}$
7.10e-29***
 & 0.0006*** %0.000624
 & & — & —  \\

\hline

% & \multicolumn{2}{c}{E2} & \multicolumn{2}{c}{E4} \\
 %\cmidrule(l){2-5}
% Sub-header row
 \textbf{Our TraFaultDia v.s.} & E2& 5-shot & 10-shot & E4 & 5-shot & 10-shot\\
 \midrule
GluAE+TEMAML &  & 0.0006*** &6.95e-28*** & & 1.70e-27*** & 9.15e-27*** \\
AttenAE+CnnMAML & &6.65e-07*** & 0.0003*** & & 2.01e-10*** & 0.176 \\
%Linear-AE +TE-MAML & 0.0742  & 0.0985  & 0.0731 & 0.0970  \\
AttenAE+NNeighbor & &1.11e-05*** & 0.1752  & & —  & —   \\
\hline
\end{tabular}
\begin{center}
\footnotesize
***p < 0.001; **p < 0.01; *p < 0.05
\end{center}
\end{table}

\begin{table}[!ht]
\centering
\small
\caption{Effect size: Cohen's d values comparing Our framework to effective baselines}
\label{tab:effectSize}
\begin{tabular}{p{3cm} | p{0.35cm} p{1cm}  p{1.2cm} | p{0.35cm} p{1cm} p{1.1cm}}
\toprule
% Header row
 %& \multicolumn{2}{c}{E1} & \multicolumn{2}{c}{E3} \\
 %\cmidrule(l){2-5}
% Sub-header row
\textbf{Our framework v.s.} & E1 & 5-shot & 10-shot & E3 & 5-shot & 10-shot\\ \midrule 
 
GluAE+TEMAML & & 0.36 & 0.13 & & 0.58 & -1.06  \\
LinearAE+TEMAML & & 1.71 & 1.35 & & 1.42 & 0.79 \\
AttenAE+NNeighbor & & 3.18  & 0.71  & & — & —  \\

\midrule

% & \multicolumn{2}{c}{E2} & \multicolumn{2}{c}{E4} \\
 %\cmidrule(l){2-5}
% Sub-header row
 \textbf{Our framework v.s.} & E2& 5-shot & 10-shot & E4 & 5-shot & 10-shot\\
 \midrule
GluAE+TEMAML & &0.71  & 3.07 & & 3.04 & 2.88  \\
AttenAE+CnnMAML & &1.06 & 0.75 & & 1.42 & 0.27 \\
%Linear-AE +TE-MAML & 0.0742  & 0.0985  & 0.0731 & 0.0970  \\
AttenAE+NNeighbor & &0.93 & 0.27  & & —  & —   \\\hline
\end{tabular}
\end{table}

\begin{table*}[!ht]
\centering
\tiny
\caption{Comparison of our framework and baselines on Trainticket.}
\label{tab:Trainticket_Result}
\begin{tabular}{l l l l l}
\toprule
% Header row
Model & \multicolumn{2}{c}{E1. TrainTicket to TrainTicket} & \multicolumn{2}{c}{E3. OnlineBoutique to TrainTicket} \\
 \cmidrule(l){2-5}
% Sub-header row
& 5-shot & 10-shot & 5-shot & 10-shot \\
\midrule
\textbf{Our MultiHAttenAE+TE-MAML} & 92.91$\pm$2.10 (74.67-100.0) & 93.26$\pm$1.40 (76.00-100.0) & 86.35$\pm$2.00 (70.67-100.0) & 92.19$\pm$1.99 (74.67-100.0)\\
\textit{MultiHAttenAE alternatives:}& & & & \\
\textbf{OnlySpan}+TE-MAML & 80.64$\pm$2.84 (57.33-97.33) &  78.77$\pm$2.80 (60.00-97.33) & 79.25$\pm$2.89 (57.33-97.33) & 80.19$\pm$3.10 (56.00-97.33)\\
% ... 其他行 ...
\textit{Multihead atten fusion alternatives:}& & & & \\
\textbf{Linear-AE}+TE-MAML &  89.15$\pm$2.29  (73.33-100.0)&  90.59$\pm$2.43 (70.67-100.0) &    83.09$\pm$2.55 (62.67-97.33) & 90.61$\pm$2.01  (72.00-100.0) \\
\textbf{GLU-AE }+TE-MAML & 92.21$\pm$1.73  (77.33-100.0) & 93.07$\pm$1.64 (77.33-100.0) & 85.07$\pm$2.38 (66.67-100.0) & 94.40$\pm$2.19 (72.00-100.0)  \\

%92.21$\pm$1.73  (77.33-100.0) & 93.07$\pm$1.64 (77.33-100.0) & 85.07$\pm$2.38 (66.67-100.0) & 94.40$\pm$2.19 (72.00-100.0)  \\

\textit{Transformer encoder alternatives:}& & & & \\
 MultiHAttenAE+\textbf{Linear-MAML} &  45.84$\pm$2.21 (25.33-61.33) &  45.36$\pm$2.16 (30.67-60.00)& 43.81$\pm$1.99 (28.00-58.67) &  43.87$\pm$1.93 (29.33-60.00) \\
 MultiHAttenAE+\textbf{RNN-MAML}  & 49.65$\pm$2.09 (37.33-64.00) & 42.88$\pm$1.93 (24.00-58.67) & 48.45$\pm$1.75 (38.67-65.33) & 47.07$\pm$1.88 (34.67-58.67)\\
 MultiHAttenAE+\textbf{LSTM-MAML}  & 41.39$\pm$2.20 (21.33-56.00) & 42.67$\pm$1.91 (29.33-56.00)  & 40.32$\pm$1.68 (22.67-52.00) & 42.29$\pm$1.79 (25.33-56.00)  \\
 MultiHAttenAE+\textbf{CNN-MAML}  & 57.06$\pm$2.85 (41.33-81.00) & 69.20$\pm$2.19 (56.00-88.00) & 49.04$\pm$1.80 (38.67-64.00) & 69.47$\pm$2.65 (48.00-89.33)\\ 

\textit{MAML alternatives:}& & & & \\
MultiHAttenAE+\textbf{TE-MatchingNet}  & 76.56$\pm$2.80 (49.33-93.33) & 76.05$\pm$2.37 (50.67-94.67) & — & —  \\
MultiHAttenAE+\textbf{ProtoNe}t & 57.25$\pm$0.03 (40.00-74.67) & 59.68$\pm$0.03 (44.00-76.00) & — & —   \\
MultiHAttenAE+\textbf{NearNeighbor} & 88.19$\pm$0.02 (74.67-98.67) & 92.56$\pm$0.02 (78.00-100.0) & — & —  \\
%MultiHAttenAE+\textbf{RelationNet}  &  &  &  &   \\
MultiHAttenAE+\textbf{DecisonTree}  & 66.80$\pm$0.03 (46.67-88.00) & 77.09$\pm$0.03 (54.67-96.00) & — & —   \\

\bottomrule
\end{tabular}
\end{table*}


\noindent\textbf{Adaptation efficiency.} Table~\ref{tab:evaluation_result_adaptability} compares the average time (in seconds) taken by our framework and the top three effective baselines to adapt to a single meta-testing task in each experiment. Our framework achieves the fastest adaptation times among all frameworks in E1 and E3 in both 5-shot and 10-shot setups. In E2, for both the 5-shot and 10-shot setups, our framework takes around 6 times less adaptation time than "AttenAE+NNeighbor", which requires immediate training of NNeighbor on new tasks' support instances before adapting to this task's query instances for evaluation.
This adaptation time difference would increase significantly as the number of various abnormal trace classification tasks grows in real-world MSS. As the number of abnormal trace classification tasks increases, the time required for NNeighbor to train on different tasks' example instances can accumulate, leading to significantly longer adaptation times than our framework. Besides, we calculate the average time our AttenAE takes to construct trace representations for each meta-testing task in our experiments and compare it with other trace representation construction approaches in the baselines. The results are presented in Table \ref{tab:trace_cons_effi}. Our AttenAE, GluAE, LinearAE require similar amounts of time to construct trace representations. %OnlySpan stands out as it takes only half the time compared to these approaches because it completely omits logs in trace representation construction, although it performs with approximately 10\% lower average accuracy in most setups of Experiments E1 to E4 compared to the other methods. 
OnlySpan stands out as it takes only half the time compared to the other approaches because it completely omits logs in trace representation construction; however, OnlySpan performs with approximately 10\% lower average accuracy in E1 to E4 setups compared to the other approaches (Table \ref{tab:E1_Result}-\ref{tab:E4_Results}).

\begin{table}[!ht]
\centering
\small
\caption{Adaptation efficiency (task average in seconds)}
\label{tab:evaluation_result_adaptability}
\begin{tabular}{p{2.8cm} | p{0.35cm} p{1cm}  p{1.2cm} | p{0.35cm} p{1cm} p{1.1cm}}
\toprule
% Header row
% & \multicolumn{2}{c}{E1} & \multicolumn{2}{c}{E3} \\
 %\cmidrule(l){2-5}
% Sub-header row
 & E1 & 5-shot & 10-shot & E3 & 5-shot & 10-shot\\
 \midrule
\textbf{Our framework} & & 0.0460 & 0.0680 & & 0.0651 & 0.0953   \\
GluAE+TEMAML & & 0.0640 & 0.0942 && 0.0651 & 0.0954  \\
LinearAE+TEMAML & & 0.0748 & 0.0946 && 0.0640 & 0.0944 \\
AttenAE+NNeighbor & & 0.1860  & 0.1890  &&  — & —  \\

\midrule

 %& \multicolumn{2}{c}{E2} & \multicolumn{2}{c}{E4} \\
 %\cmidrule(l){2-5}
% Sub-header row
 & E2& 5-shot & 10-shot & E4 & 5-shot & 10-shot\\
 \midrule
\textbf{Our framework} & & 0.0848 & 0.0977 & & 0.0875 & 0.0974   \\
GluAE +TEMAML & &0.0801  & 0.0978 &  &0.0731 & 0.0969  \\
CnnMAML & & 0.0470 & 0.0472 & & 0.0417 &0.0490 \\
%Linear-AE +TE-MAML & 0.0742  & 0.0985  & 0.0731 & 0.0970  \\
AttenAE+NNeighbor & & 0.5140 & 0.5307   && —  & —   \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\end{table}

\begin{table}[!ht]
\centering
\small
\caption{Trace construction efficiency (task average in seconds)}
\label{tab:trace_cons_effi}
\begin{tabular}{p{2.3cm}|lll|lll}
\toprule
% Header row
 %& \multicolumn{2}{c}{Trainticket} & \multicolumn{2}{c}{OnlineBoutique} \\
 %\cmidrule(l){2-5}
% Sub-header row
 & TrainTicket & 5-shot & 10-shot & OnlineBoutique& 5-shot & 10-shot\\\hline
\textbf{Our AttenAE} & & 1.8436 & 2.1524  & & 4.1426 & 5.0189 \\
GluAE && 1.8395  & 2.1541 && 4.3121 & 5.1921  \\
LinearAE && 1.8286  & 2.1486 && 4.1223 & 5.2066 \\
OnlySpan && 1.1671 & 1.1818 && 1.9065 & 2.1822  \\

%1.5436 1.8524
\bottomrule
\end{tabular}
\end{table}

\noindent \textbf{Answers to our research questions:} The above evaluation results
indicate that, compared to the other baselines, our framework demonstrates more robust adaptation effectiveness with more feasible adaptation efficiency. Thus, we conclude that, our framework demonstrates effective and efficient within-system and cross-system adaptability, making it a promising approach for classifying (multi-class classification) abnormal traces into precise fault types for MSS.  


\subsection{Ablation study} As shown in Table \ref{tab:E1_Result}-\ref{tab:E4_Results}, each component of our framework contributes to its overall effectiveness, with AttenAE is the most significant contributor. The impact of AttenAE is evident from these tables, where our framework consistently outperforms  the AttenAE alternative ``OnlySpan+TEMAML" by approximately 10\% in E1 to E4 setups. Additionally, we conduct an ablation study on the number of meta-learning tasks to train TEMAML. Our current study uses 4 meta-training tasks in our experiments.  We tested 2-4 meta-training tasks and found that using 4 meta-training tasks yielded the best average accuracy across 50 meta-testing tasks in each experiment, see Table \ref{tab:Ablation_meta_traning_tasks}. This result aligns with the nature of MAML as a multi-task learning algorithm: including more varied meta-training tasks can enhance the algorithm's robustness, improving its ability to adapt to new, unseen tasks across different contexts.

% \begin{table}[!ht]
% \centering
% \caption{Ablation study on the number of normal traces to train AttenAE}
% \label{tab:ablation_normal_trace}
% \begin{tabular}{p{2.2cm} p{1cm} p{1.2cm} p{1cm} p{1.1cm} p{1cm} p{1.1cm} p{1cm} p{1.1cm}}
% \toprule
% % Header row
%  & \multicolumn{2}{c}{E1} & \multicolumn{2}{c}{E2} & \multicolumn{2}{c}{E3} & \multicolumn{2}{c}{E4}  \\
%  \cmidrule(l){2-9}
% % Sub-header row
%  &  5-shot & 10-shot & 5-shot & 10-shot & 5-shot & 10-shot & 5-shot & 10-shot\\
%  \midrule
% \textbf{Current: 3960} & 92.91 & 93.26 &  &  & 86.35 & 92.19 & 82.37 & 84.77 \\
% 2/3 of current & 73.17 & 74.67 & 0.0651 & 0.0954 & 75.40 & 77.00 &\ \\
% 1/3 of current & 69.60& 75.50 & 0.0954 & & 69.07 & 70.67\\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[ht]
\centering
\small
\caption{Ablation study on the number of meta-training tasks in TEMAML}
\label{tab:Ablation_meta_traning_tasks}
\begin{tabular}{p{2.2cm} p{1cm} p{1.2cm} p{1cm} p{1.1cm} p{1cm} p{1.1cm} p{1cm} p{1.1cm}}
\toprule
% Header row
  & \multicolumn{2}{c}{E1} & \multicolumn{2}{c}{E2} & \multicolumn{2}{c}{E3} & \multicolumn{2}{c}{E4}  \\
 \cmidrule(l){2-9}
% Sub-header row
 N of tasks &  5-shot & 10-shot & 5-shot & 10-shot & 5-shot & 10-shot & 5-shot & 10-shot\\
 \midrule
\textbf{Current: 4} & 92.91 & 93.26 & 82.50 & 85.20 & 86.35 & 92.19 & 82.37 & 84.77 \\
3 & 89.67  & 91.00 & 80.53 & 82.13 & 85.03 & 89.07 & 81.92 & 82.67\\
2 & 88.17 & 89.33 & 78.67 & 78.10 & 83.11 & 85.78 & 74.67 & 77.33 \\
\bottomrule
\end{tabular}
\vspace{-15pt}
\end{table}





